Multiagent Inverse Reinforcement Learning via Theory of Mind Reasoning

We approach the problem of understanding how people interact with each other in collaborative settings, especially when individuals know little about their teammates, via Multiagent Inverse Reinforcement Learning (MIRL), where the goal is to infer the reward functions guiding the behavior of each individual given trajectories of a team's behavior during some task. Unlike current MIRL approaches, we do not assume that team members know each other's goals a priori; rather, that they collaborate by adapting to the goals of others perceived by observing their behavior, all while jointly performing a task. To address this problem, we propose a novel approach to MIRL via Theory of Mind (MIRL-ToM). For each agent, we first use ToM reasoning to estimate a posterior distribution over baseline reward profiles given their demonstrated behavior. We then perform MIRL via decentralized equilibrium by employing single-agent Maximum Entropy IRL to infer a reward function for each agent, where we simulate the behavior of other teammates according to the time-varying distribution over profiles. We evaluate our approach in a simulated 2-player search-and-rescue operation where the goal of the agents, playing different roles, is to search for and evacuate victims in the environment. Our results show that the choice of baseline profiles is paramount to the recovery of the ground-truth rewards, and that MIRL-ToM is able to recover the rewards used by agents interacting both with known and unknown teammates.

==> Sections/response.tex <==
We would like to thank the reviewers for the feedback. The comments are very helpful in improving our paper in terms of content and readability, for which we are deeply grateful.


Response to Questions:

Reviewer 1 Q1: The significance of FC Diff was explained in the last paragraph of Page 7. "The Profile columns correspond ... using a fixed Gt model of the teammate (no ToM)." We expect the range of this metric to be from 2.38 to 30.55 for agent Medic and from 2.25 to 14.84 for agent Explorer with the Monte Carlo sample size 16. The MILR cond-1 column represents the best FC diff using decentralized learning with ground truth reward models. The significance of our algorithm can be shown by evaluating how small the FC diff is and how far it deviates from the FC diff of using Op profile.

Reviewer 1 Q2: As our approach is extended from MaxEnt IRL, it finds the trajectory that is exponentially preferred among a distribution of trajectories. A larger sample size of trajectories would definitely help the convergence but dramatically increases the computation. We empirically experimented the number of demonstration (16), trajectory length (25 steps) and trajectory sample size (16), and verified its convergence in FC diff with different random seeds as shown in column Profile-Gt of Table 4. We could expect that the FC Diff would approach to 0 with more demonstrations and samples. This is also why we consider the small but not 0 FC Diff of MIRL-ToM as good convergence.

Reviewer 3
- Pg3 Sec3.2: We have clarified the definition of feature count by adding "MaxEnt IRL considers the trajectory reward R(zeta) as a linear combination of feature counts (i.e., R(zeta)=theta T phi(zeta))", where "theta" is the reward model parameters. The equation of "theta*" states the learning objective function of IRL.

- Pg4 Sec4: The goal of the team is to reach the ultimate state of the task (i.e., "evacuate all victims" in search-and-rescue tasks); the intention of an agent can be understood as the decision-making based on rewards at a state or the subgoals in the task; profiles are the different reward models an agent can have. This paragraph serves as the preliminary introduction to our modeling and methods. Section 4.1, 4.2 formulate reward models, action/policy, and learning method. Section 5.1 specifies an search-and-rescue task with detailed list of reward features (goals/intentions) and reward models such as Gt, Op, Tk, Sc (profiles).

- Pg4 Sec4.2: We have clarified this by changing "motivations" to "models" since an agent makes a decision based on the expected models of its teammates.

- Pg5 Sec5.1: We have clarified this by changing the sentence to "n locations, where each location has an information state..." since each location provides additional information on victim status.

- Pg5, Table1: A reward function is a linear combination of reward features parameterized by the weights.we have changed the table caption to "reward functions of features "phi" and weights "theta"" to avoid confusions.

- Pg 6 Fig5: Due to the limited space, we cannot use two columns to show the plots, but we have enlarged and color-coded the actions of two agents.

- Pg4 Sec4.1 and Pg6 Sec5.3: We have fixed these typos.


Plans for Improvement before Final Version:
- Related work: We will enhance the related work section by comparing more studies on Theory of Mind and Multi-agent IRL in addition to the articles suggested by Reviewer 1.

- 2 agents in 3x3 gridworld: Although the task only involves 2 agents in 9 locations, it is challenging because of the following three aspects:
1) Each grid has an information state on victim status in addition to location coordinates, and there are multiple possible status from unknown to clear, making the state space grow exponentially.
3) The action space for each agent is larger than just 4-way movement, and the task requires the coordination of agents, allowing us to model various profiles of agents. With theory of mind, one agent is interacting with the profiles of the other agent, making the problem harder.
2) The fact that there are less steps needed for task completion in the 3x3 gridworld makes the model inference phase much more challenging since agents would be uncertain about each other for the most steps.

We will clarify these challenges when introducing the experiment and encourage computation advancement in future works.


Sincerely,
the authors
